DF-Net: Unsupervised Joint Learning of Depth and Flow using Cross-Task Consistency

We present an unsupervised learning framework for simultaneously training single-view depth prediction and optical flow estimation models using unlabeled video sequences. Existing unsupervised methods often exploit brightness constancy and spatial smoothness priors to train depth or flow models. In this paper, we propose to leverage geometric consistency as additional supervisory signals. Our core idea is that for rigid regions we can use the predicted scene depth and camera motion to synthesize 2D optical flow by backprojecting the induced 3D scene flow. The discrepancy between the rigid flow (from depth prediction and camera motion) and the estimated flow (from optical flow model) allows us to impose a cross-task consistency loss. While all the networks are jointly optimized during training, they can be applied independently at test time. Extensive experiments demonstrate that our depth and flow models compare favorably with state-of-the-art unsupervised methods.

==> acknowledgement.tex <==
\section*{Acknowledgement}
\label{sec:acknowledgement}

This work was supported in part by NSF under Grant No. (\red{XXX}). We gratefully acknowledge the support of NVIDIA Corporation with the donation of the Titan Xp GPU.
%

==> overview.tex <==
\input{figure/fig_overview}

\section{Overview}
\label{sec:overview}

Here we present an unsupervised adaptation framework for jointly improving the single-view depth network and the optical flow network using unlabeled video sequences. The overall pipeline is shown in Figure~\ref{fig:model}, given two consecutive frames $(I_t, I_{t+1})$ from unlabeled video, we estimate depth of frame $I_t$, and optical flow from frame $I_t$ to $I_{t+1}$. We also need to estimate the camera pose transformation, which can be done with any visual odometry or SLAM system. Here we use a CNN module to achieve this. Then, we can synthesize the 3D scene flow with the estimated depth and pose~(Sec. \ref{sec:synthesis}), and backproject it as 2D flow, which we refer as "DP flow" in this paper. Suppose most of the object transformation in these video sequences can be explained by camera motion, i.e. the scenes are mostly static, then the "DP flow" should be consistent with estimated optical flow. However, if we train the depth network and flow network separately, there is no guarantee to be consistent with each other. Hence, we propose a geometry-aware cross-network consistency as additional supervision signal, to fine-tune and improve the two branches (Sec. \ref{sec:consistency}). We also propose an heuristic trick to handle the non-rigid transformation, which cannot be explained by the camera motions.

